MemLLM: Finetuning LLMs to Use An Explicit Read-Write Memory

While current large language models (LLMs) perform well on many knowledge-related tasks, they are limited by relying on their parameters as an implicit storage mechanism. As a result, they struggle with memorizing rare events and with updating their memory as facts change over time. In addition, the uninterpretable nature of parametric memory makes it challenging to prevent hallucination. Model editing and augmenting LLMs with parameters specialized for memory are only partial solutions. In this paper, we introduce MemLLM, a novel method of enhancing LLMs by integrating a structured and explicit read-and-write memory module. MemLLM tackles the aforementioned challenges by enabling dynamic interaction with the memory and improving the LLM's capabilities in using stored knowledge. Our experiments indicate that MemLLM enhances the LLM's performance and interpretability, in language modeling in general and knowledge-intensive tasks in particular. We see MemLLM as an important step towards making LLMs more grounded and factual through memory augmentation. The project repository is publicly available at https://github.com/amodaresi/MemLLM

==> figures/memllm.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth, trim=3 3 3 3, clip] {figures/files/MEMLLM_vs_PLM.pdf}
    \caption{A vanilla pretrained LLM can produce
      hallucinated nonfactual output. In contrast,
      \framework dynamically queries its explicit memory for
      stored facts, resulting in more factually grounded text generation.}
    \label{fig:memllm_vs_plm}
\end{figure}


==> tables/memory_read.tex <==
\begin{table*}[t]
	\small
	\setlength\tabcolsep{3pt}
	\centering
	\begin{tabular}{lccc}
		\toprule
         & \multicolumn{3}{c}{\textbf{PPL}} \\
		 & \textbf{Overall} &\textbf{Target} & \textbf{All} \\
		\midrule
        Baseline \#1 (Mistral-7b) & 1.774 & 1.180 & 1.420 \\
        Baseline \#2 (Mem. Disabled) & 1.616 & 1.151 & 1.355 \\
        \midrule
        \multicolumn{4}{c}{Memory: MW[\emph{Wikipedia (Full)}]}\vspace{3pt} \\
        \circled{1} \textbf{\framework} & 1.606 & 1.009 & 1.322 \\
		% \qquad + Gold MR Position & 1.602 & 1.007 & 1.316 \\
        % \qquad + Gold Queries & 1.598 & 0.901 & 1.287 \\
        % \qquad + Gold Target & 1.535 & 0.337 & 1.124 \\
        \midrule
        \multicolumn{4}{c}{Memory: MW[\emph{Wikipedia (Abs.)}]}\vspace{3pt} \\
        \circled{2} \framework & 1.607 & 1.013 & 1.324 \\
        % \midrule
        % \multicolumn{4}{c}{Memory: MW[\emph{DOCRED(Val.)}]}\vspace{3pt} \\
        % \framework & 1.594 & 0.963 & 1.300 \\
        \midrule
        \multicolumn{4}{c}{Memory: MW[\emph{Re-\docred (Test)}]}\vspace{3pt} \\
        \circled{3} \framework & 1.589 & 0.945 & 1.289 \\
        \qquad \circled{4} + Gold MR Pos. \& Queries & 1.578 & 0.786 & 1.287 \\
        \midrule
        \multicolumn{4}{c}{Memory: Re-\docred (Test)}\vspace{3pt} \\
        \circled{5} \framework & 1.589 & 0.913 & 1.290 \\
        \qquad \circled{6} + Gold MR Position & 1.579 & 0.847 & 1.268 \\
        \qquad \circled{7} + Gold Queries & 1.562 & 0.619 & 1.202 \\
        \qquad \circled{8} + Gold Target & 1.544 & 0.448 & 1.152 \\
        \qquad \circled{9} + Gold Target Only & 1.535 & 0.337 & 1.124 \\
        % \qquad + Gold MR Pos. \& Queries & 1.562 & 0.619 & 1.202 \\
    % \midrule
    % \multicolumn{5}{c}{\emph{Without late stopping}}\vspace{3pt} \\
		% Distant. & 0.541 & 0.325 & 0.587 & 0.563 \\
    % \qquad w/ Filtering + 85\% NoRel. Drop + 10xAnnot. & 0.562 & \textbf{0.448} & \textbf{0.818} & 0.666 \\
		\bottomrule
	\end{tabular}
	\caption{\framework performance in terms of perplexity of overall (whole) text, target and all entities. The effect of changing the memory content to other sources has been demonstrated. Memories labeled as "MW[\emph{X}]" are populated with relations generated through memory-writes using documents from source \emph{X}. Otherwise, the relations are directly from the stated split of Re-\docred.}
	\label{tab:memory_read_PPLs}
\end{table*}

